Safe Reinforcement Learning with Hard Constraints: Policy Gradient Methods with Intersample Guarantees

We develop a policy-gradient (PG) reinforcement learning (RL) framework with hard inter-sample control barrier function (CBF)-based safety constraints for nonlinear sampled-data systems. We first design a class of stochastic policies with support truncated to sampling-period-dependent safe control sets, that guarantee safety-by-construction at sampling instants. We then propose a model-free PG algorithm that searches over the class of safe-by-design policies and establish sufficient conditions on sampling-period such that any action sampled from safe control sets remains safe throughout the sampling interval, providing inter-sample guarantees. We further establish finite-time convergence and sample complexity guarantees for the proposed PG algorithm and characterize its global optimality under gradient dominance. Finally, we illustrate inter-sample safety guarantees on a safe quadrotor navigation environment.

==> experiments.tex <==
\section{Safe Quadrotor Experiment}
\label{sec:safe_quadrotor_experiment}
\color{black}
We evaluate \texttt{SASPG} on the quadrotor navigation setup
in~\cite{suttle2024sampling,sharma2026safepg}.
From the small-angle model
in~\cite{suttle2024sampling}, we consider the continuous-time quadrotor dynamics as
\begin{equation}\label{eq:quad-continuous}
 \dot p=v,\qquad \dot v=u,
\end{equation}
where $x=(p^\top,v^\top)^\top\in\R^4$ contains $x-y$ plane position
and velocity, and $u\in\U_{\mathrm{act}}=[-4,4]^2\,\mathrm{m/s^2}$
is the acceleration. The task is to reach
$p_{\mathrm g}=(15,15)\,\mathrm m$ from initial position
$p_0=(-1.5,-1.5)\,\mathrm m$ while avoiding an obstacle
centered at $(6.75,6.75)\,\mathrm m$. For safety, we model collision avoidance with $h(p)\ge0$, where CBF $h$ is given as
\begin{equation}\label{eq:quad_obstacle}
 h(p)=\left(\frac{p_x-6.75}{4}\right)^4
     +\left(\frac{p_y-6.75}{3}\right)^4-\tfrac12.
\end{equation}
We use the relative-degree-two barrier expression
$\psi=\ddot h+8\dot h+6h$~\cite{sharma2026safepg}.
Applying the margin construction~\eqref{eq:SASafeSet} with
$\underline\psi=\psi$ gives the sampling-aware safe control set
\begin{equation}\label{eq:quad-safe-set}
 \widehat{\mathcal C}_\delta(x)
 =\{u\in\U_{\mathrm{act}}:\psi(x,u)\ge\delta M_\psi(x,\delta)\},
\end{equation}
where $M_\psi(x,\delta)$ bounds $|\dot\psi|$ over a hold,
ensuring $\psi\ge0$ between updates. We use
$\delta=0.10\,\mathrm s$ and verify the
pointwise feasibility criterion underlying
Proposition~\ref{prop:period},
$\delta M_\psi(x,\delta)<\max_{u\in\U_{\mathrm{act}}}\psi(x,u)$,
at each executed evaluation update. Under~\eqref{eq:zoh}, the
exact sampled-data dynamics are
\begin{equation}\label{eq:quad-sampled}
 p_{k+1}=p_k+\delta v_k+\tfrac12\delta^2u_k,\quad
 v_{k+1}=v_k+\delta u_k.
\end{equation}
We use the base policy
$\pi_\theta(\cdot\mid\xi)=\mathcal N(\mu_\theta(\xi),0.25I_2)$
centered around a PI controller~\cite{sharma2026safepg}, with $\theta=(k_p,k_i)$ and
observation $\xi=(p,v,I)$, given by
\begin{equation}\label{eq:quad-mean}
 \mu_\theta(\xi)=k_p(p_{\mathrm g}-p)+k_iI-0.85v,
\end{equation}
Here, $I\in\R^2$ is a clipped,
exponentially weighted integral of the position error
$p_{\mathrm g}-p$.

For efficient sampling, we approximate $\widehat{\mathcal C}_\delta(x)$ with a maximum-area inner rectangle following~\cite{suttle2024sampling} and its
implementation~\cite{sharma2024cbfrepo}. Then, we obtain the safe-by-design policy $\pi_\theta^{\delta}$
from~\eqref{eq:policy}, and run
Algorithm~\ref{alg:safegrad} with return \eqref{eq:rl-return}, $\gamma=0.99$ and per-step reward
\begin{equation}
 r(p,u)=-\min\left\{\frac{\|p_{\mathrm g}-p\|_2}{20},1\right\}
        -\frac{0.01}{32}\|u\|_2^2.
\end{equation}
Using Algorithm~\ref{alg:SASPG}, we train ten policies for 500
updates each with batch size eight. We procide further implementation and evaluation details in Appendix~\ref{app:proofs}, item~(\ref{app:experiment-details}).
We show in Figure~\ref{fig:quad_safe_navigation} that \texttt{SASPG} learns a safe quadrotor navigation policy that is safe throughout operation. 
% Among 1,000 held-out trials with a
% $40\,\mathrm s$ evaluation window, 998 reach the goal and two
% time out, with no observed collisions or infeasible stops.
\begin{figure}[!htb]
 \centering
 \includegraphics[width=\columnwidth,height=0.30\textheight,keepaspectratio]{images/navigation.pdf}
 \caption{\texttt{SASPG} navigation around the central obstacle.
 Twenty held-out rollouts are shown in light blue; the bold curve
 is the median-length successful rollout of the representative controller.}
 \label{fig:quad_safe_navigation}
\end{figure}
% We audit safety at the endpoints and all real critical points
% of each held-input barrier polynomial.


==> proofs.tex <==
\section{Proofs and Experimental Details}

\label{app:proofs}

\begin{enumerate}[label=(\roman*),ref=\roman*,leftmargin=0pt,itemindent=2em,labelwidth=1.5em,labelsep=0.5em,itemsep=6pt,topsep=0pt]

\item\label{app:proof-safety}\textbf{Proof of Theorem~\ref{thm:safety}.}
For $x_k\in\Ssafe$ and $u_k\in\Cdel(x_k)$,
Assumption~\ref{ass:safety} and~\eqref{eq:SASafeSet} imply, for
$0\le s\le\delta$,
\begin{equation}\label{eq:lower}
\begin{aligned}
 \psi(x(k\delta+s),u_k)
 &\ge\underline\psi(x_k,u_k)-M_\psi s\\
 &\ge M_\psi(\delta-s)\ge0.
\end{aligned}
\end{equation}
Hence $\dot h(x(t))+\alpha_1(h(x(t)))\ge0$ almost everywhere on
$[k\delta,(k+1)\delta]$. Scalar comparison preserves $h(x(t))\ge0$
from $h(x_k)\ge0$. Induction over the sampling intervals proves
forward invariance of $\Ssafe$, and the uniform existence condition
permits continuation at each update. The actuator constraints follow
from $\Cdel(x_k)\subseteq\U_{\mathrm{act}}$.\hfill\(\square\)\par


\item\label{app:proof-period}\textbf{Proof of Proposition~\ref{prop:period}.}
We show $\lambda_m(\Cdel(x))>0$ for every $x\in\Ssafe$.
By definition, $m_{\mathrm{act}}=\inf_{x\in\Ssafe}
\max_{u\in\U_{\mathrm{act}}}\underline\psi(x,u)$.
For each $x\in\Ssafe$, continuity of $\underline\psi(x,\cdot)$ and
compactness of $\U_{\mathrm{act}}$ give a maximizing input $u^\star$
with $\underline\psi(x,u^\star)\ge m_{\mathrm{act}}>M_\psi\delta$.
Continuity preserves this strict inequality in a neighborhood of
$u^\star$ within the actuator box. Since the box has nonempty interior,
this neighborhood has positive volume and belongs to $\Cdel(x)$.\hfill\(\square\)\par


\item\label{app:proof-smoothness}\textbf{Proof of Lemma~\ref{lem:score}.}
Assumption~\ref{ass:policy}(\ref{asum-item-integrability})
justifies differentiation of the normalizer and finite-horizon
trajectory expectations. Since $\Cdel(x)$ is
independent of $\theta$, differentiating the normalizer gives
$\nabla_\theta\log Z_\theta^\delta(x)
=\E_{v\sim\pdel(\cdot\mid x)}[b_\theta(x,v)]$,
which yields~\eqref{eq:score}.
Set $G:=\sqrt{2\mathsf S_2}$ and $H_s:=\mathsf H_1$.
For a reward $r_k=r(x_k,u_k)$, write
$S_k=\sum_{i=0}^k s_\theta^\delta(x_i,u_i)$ and
$T_k=\sum_{i=0}^kD_\theta s_\theta^\delta(x_i,u_i)$.
Finite-horizon likelihood differentiation gives
$\nabla_\theta^2\E_\theta^\delta[r_k]
=\E_\theta^\delta[r_k(S_kS_k^\top+T_k)]$.
The moment conditions imply
$\E_\theta^\delta[\norm{S_k}^2]\le(k+1)^2G^2$ and
$\E_\theta^\delta[\norm{T_k}]\le(k+1)H_s$. Hence
\[
 \norm{\nabla_\theta^2\E_\theta^\delta[r_k]}
 \le\bar r[(k+1)^2G^2+(k+1)H_s].
\]
Also,
$\norm{\nabla_\theta\E_\theta^\delta[r_k]}
\le\bar r(k+1)\sqrt{\mathsf S_2}$.
After multiplication by $\gamma^k$, both bounds are summable uniformly
in $\theta$, justifying differentiation of the infinite-horizon return.
Using
$\sum_{k\ge0}\gamma^k(k+1)^2=(1+\gamma)/(1-\gamma)^3$
and $\sum_{k\ge0}\gamma^k(k+1)=(1-\gamma)^{-2}$
in the Hessian bound yields~\eqref{eq:L}.
The gradient inequality follows by integration along the segment
joining $\theta$ and $\theta'$.\hfill\(\square\)\par


\item\label{app:proof-estimator}\textbf{Proof of Lemma~\ref{lem:variance}.}
Fix $\theta$ and let $K\sim\Geom(1-\gamma)$ be independent
of the reset state and rollout. Then
\[
 \mathcal L_\theta^\delta(x_K)
 =(1-\gamma)\sum_{k=0}^{\infty}
       \gamma^k\mathcal L_\theta^\delta(x_k)
 =d_\theta^\delta.
\]
At $x=x_K$, draw $u,v$ conditionally independently from
$\pdel(\cdot\mid x)$ and set
$A_\theta(x,u,v)=b_\theta(x,u)-b_\theta(x,v)$.
By~\eqref{eq:score},
\[
 \E[A_\theta(x,u,v)\mid x,u]=s_\theta^\delta(x,u).
\]
With $q=\sqrt\gamma$ and an independent $H\sim\Geom(1-q)$,
the randomized return satisfies
\begin{equation}\label{eq:Qhat}
 \widehat Q_\delta=\sum_{h=0}^H q^h r_h,
 \qquad |\widehat Q_\delta|\le\frac{\bar r}{1-q}.
\end{equation}
Since $\Pr(H\ge h)=q^h$ and $q^2=\gamma$, bounded rewards
allow interchange of expectation and summation, giving
$\E[\widehat Q_\delta\mid x,u]=Q_\theta^\delta(x,u)$.
Conditional independence of $v$ and the return continuation then gives
\[
 \E[\widehat Q_\delta A_\theta(x,u,v)\mid x,u]
 =Q_\theta^\delta(x,u)s_\theta^\delta(x,u).
\]
Equation~\eqref{eq:pg} proves unbiasedness.
The paired-score second moment is
\begin{equation}\label{eq:pair-moment}
\begin{aligned}
 \E[\norm{A_\theta(x,u,v)}^2\mid x]
 &=2\E[\norm{s_\theta^\delta(x,u)}^2\mid x]\\
 &\le2\mathsf S_2.
\end{aligned}
\end{equation}
Together with~\eqref{eq:Qhat}, this gives
$\E[\norm{\widehat g_\delta}^2]\le V_\delta$, and hence the variance bound.

The first stage applies $K$ inputs, and the second applies
$H+1$ inputs, including the initial action $u$.
The auxiliary action $v$ is not applied to the plant.
Since $0<\gamma,q<1$, both stopping times are finite almost surely.
Their geometric distributions give
$\E[K]=\gamma/(1-\gamma)$ and $\E[H+1]=1/(1-q)$,
which prove~\eqref{eq:H}. For a fixed number $N_{\rm PG}$ of
estimator calls, linearity of expectation gives
$N_{\rm PG}\mathsf H$ actuated intervals in expectation,
including when the policy parameter changes between calls.\hfill\(\square\)\par


\item\label{app:convergence-proof}\textbf{Proof of Theorem~\ref{thm:optimality}.}
Let $\mathcal F_j$ contain all randomness before batch $j$, so
$\theta_j$ is $\mathcal F_j$-measurable. Independent calls to
\textsc{SafeGrad} and Lemma~\ref{lem:variance} give
\begin{equation}\label{eq:batch}
\begin{aligned}
 \E[\overline g_j\mid\mathcal F_j]&=\nabla J_\delta(\theta_j),\\
 \E[\norm{\overline g_j-\nabla J_\delta(\theta_j)}^2
       \mid\mathcal F_j]&\le V_\delta/B.
\end{aligned}
\end{equation}
For $\eta\le L_\delta^{-1}$, smoothness and~\eqref{eq:batch} yield
\begin{equation}\label{eq:ascent}
\begin{aligned}
 \E[J_\delta(\theta_{j+1})\mid\mathcal F_j]
 &\ge J_\delta(\theta_j)
   +\frac\eta2\norm{\nabla J_\delta(\theta_j)}^2\\
 &\quad-\frac{L_\delta\eta^2V_\delta}{2B}.
\end{aligned}
\end{equation}
Define $z_j=J_\delta^*-\E[J_\delta(\theta_j)]-b_\delta$,
$c=\eta/(2a_\delta^2)$, and $d=L_\delta\eta^2V_\delta/(2B)$.
Write $[z]_+=\max\{z,0\}$.
Weak gradient dominance and Jensen's inequality imply
$\E[\norm{\nabla J_\delta(\theta_j)}^2]
\ge[z_j]_+^2/a_\delta^2$, hence
\begin{equation*}
 z_{j+1}\le z_j-c[z_j]_+^2+d.
\end{equation*}
Write $p_0=[z_0]_+$ and set
\begin{equation}\label{eq:lambda}
\begin{aligned}
 r=\xi_\eta&=a_\delta\sqrt{\frac{L_\delta\eta V_\delta}{B}},\\
 \lambda=\lambda_\eta&=cr=\frac{\eta\xi_\eta}{2a_\delta^2}.
\end{aligned}
\end{equation}
The step-size restriction~\eqref{eq:stepsize} gives
$0<\lambda\le1/2$.
For $z_j\le r$, the recursion gives $z_{j+1}\le r$:
for $z_j\le0$ use $d=\lambda r\le r$, and on $[0,r]$
use monotonicity of $z-cz^2+d$. For $z_j>r$,
\begin{equation*}
 z_j-cz_j^2+d
 =r+(1-2\lambda)(z_j-r)-c(z_j-r)^2.
\end{equation*}
Thus $[z_{j+1}-r]_+\le(1-\lambda)[z_j-r]_+$.
Iteration and $[z_0-r]_+\le p_0$ prove~\eqref{eq:gap}.

For any $\varepsilon>0$, choose
\begin{equation}\label{eq:eta}
 \eta=\min\left\{\eta_{\max},
       \frac{B\varepsilon^2}{4a_\delta^2L_\delta V_\delta}\right\},
\end{equation}
so $r\le\varepsilon/2$. Define
$\Lambda_\varepsilon=\log\max\{1,2p_0/\varepsilon\}$ and set
\begin{equation}\label{eq:iterations}
 T=\max\left\{1,
      \left\lceil\frac{\Lambda_\varepsilon}{\lambda}\right\rceil
      \right\}.
\end{equation}
Since $(1-\lambda)^T p_0\le\varepsilon/2$,
\eqref{eq:gap} gives $b_\delta+\varepsilon$ accuracy.
Also, $N_{\rm PG}=BT\le B+B\Lambda_\varepsilon/\lambda$;
substitution of~\eqref{eq:eta} gives
\begin{equation}\label{eq:complexity}
\begin{aligned}
 N_{\rm PG}\le B+\Lambda_\varepsilon\max\Biggl\{
 &\frac{2a_\delta B^{3/2}L_\delta}{\sqrt{V_\delta}},\ 2B,\\
 &\frac{16a_\delta^4L_\delta V_\delta}{\varepsilon^3}\Biggr\}.
\end{aligned}
\end{equation}
This yields the claimed small-$\varepsilon$ order for fixed $B$ and problem constants.
Equation~\eqref{eq:H} gives the expected interaction count.
\hfill\(\square\)\par


\end{enumerate}

\begin{remark}[Stationarity without weak gradient dominance]
\label{rem:stationarity}
Under Assumptions~\ref{ass:safety} and~\ref{ass:policy} and the
period condition~\eqref{eq:period}, telescoping~\eqref{eq:ascent}
yields, for $0<\eta\le L_\delta^{-1}$ and integer $T\ge1$,
\begin{equation}\label{eq:stationary}
\begin{aligned}
 \frac1T\sum_{j=0}^{T-1}\E[\norm{\nabla J_\delta(\theta_j)}^2]
 &\le\frac{2[J_\delta^*-J_\delta(\theta_0)]}{\eta T}\\
 &\quad+\frac{L_\delta\eta V_\delta}{B}.
\end{aligned}
\end{equation}
This uses smoothness,~\eqref{eq:batch}, and
$\E[J_\delta(\theta_T)]\le J_\delta^*$.
\end{remark}
%
\begin{enumerate}[label=(\roman*),ref=\roman*,start=6,leftmargin=0pt,itemindent=2em,labelwidth=1.5em,labelsep=0.5em,itemsep=6pt,topsep=0pt]
\item\label{app:experiment-details}\textbf{Experimental details.}\par
\noindent\textit{Continuous-Time Model and Sampled State.} 
Within each hold,~\eqref{eq:quad-sampled} with $\delta$ replaced
by $s\in[0,\delta]$ gives the exact flow.
We draw $p_0$ uniformly from $(-1.5,-1.5)+[-0.25,0.25]^2$
and $v_0$ from $[-0.1,0.1]^2$, with $I_0=0$. Initial states satisfy $h\ge0$ and
$\dot h+(4-\sqrt{10})h\ge0$.
The integral memory is updated by
$I_{k+1}=\operatorname{clip}(e^{-\ell\delta}I_k+
\delta(p_{\mathrm g}-p_k),-8,8)$ componentwise, where
$\ell=0.100503\,\mathrm{s^{-1}}$.
Memory, the goal timer, and the terminal mode are included in the
sampled Markov state.

\noindent\textit{Barrier Margin and Inner Rectangle.} 
Write $\rho_i=p_i-o_i$, with $o=(6.75,6.75)$ and
$(a_1,a_2)=(4,3)$. For $U=4$, let
$Q_i=|\rho_i|+\delta|v_i|+\tfrac12\delta^2U$ and
$V_i=|v_i|+\delta U$, which bound position and velocity over a hold.
Differentiating $\psi=\ddot h+8\dot h+6h$ gives
\begin{equation}\label{eq:quad-M}
 \begin{aligned}
 M_\psi(x,\delta)=\sum_{i=1}^2\frac1{a_i^4}\Bigl[
 &24Q_iV_i^3+36Q_i^2V_iU\\
 &+8(12Q_i^2V_i^2+4Q_i^3U)+24Q_i^3V_i\Bigr].
 \end{aligned}
\end{equation}
Thus $\psi(x(t_k+s),u_k)\ge\psi(x_k,u_k)-M_\psi(x_k,\delta)s$.
The affine input constraint and its maximum-area inner rectangle
follow~\cite[Appendices C.2.2--C.2.3]{suttle2024sampling}
and~\cite{sharma2024cbfrepo}, with the threshold tightened by
$\delta M_\psi$ as in~\eqref{eq:quad-safe-set}.

\noindent\textit{Gaussian Truncation and Gradient Estimates.} 
We sample the rectangle-truncated Gaussian coordinatewise by
inverse-CDF sampling, with $\sigma=0.5$.
The paired score follows from~\eqref{eq:score} using
$b_\theta=\sigma^{-2}(D_\theta\mu_\theta)^\top(u-\mu_\theta)$
and $D_\theta\mu_\theta=[p_{\mathrm g}-p\ \ I]$.
Algorithm~\ref{alg:safegrad} supplies the gradient estimates.
We initialize $(k_p,k_i)=(0.18,0)$ and use step size $10^{-4}$,
clip the averaged gradient to norm two, and project the gains
onto $[0,1]\times[0,0.1]$.

\noindent\textit{Termination and Evaluation.} 
Each controller is tested on 100 common held-out seeds for
$40\,\mathrm s$. Goal completion requires position error at most
$0.5\,\mathrm m$ and speed at most $0.3\,\mathrm{m/s}$ for one second.
Goal and failure states are absorbing, with rewards zero and
$-1.01$ per step. An infeasible set, sampling failure,
collision, or escape beyond $100\,\mathrm m$ per coordinate
terminates a trial.
Figure~\ref{fig:quad_safe_navigation} uses the controller with
lower-median mean evaluation return across the ten training seeds.
We audit $h$, $\beta=\dot h+(4-\sqrt{10})h$, and $\psi$ at
endpoints and real derivative roots in $[0,\delta]$
(collision tolerance $10^{-8}$).
\end{enumerate}


==> sections/analytical_example.tex <==
\section{Analytical Illustration}\label{sec:example}
\color{black}
Consider $\dot x=u$ with actuator magnitude limit $|u|\le a$,
so $\U_{\mathrm{act}}=[-a,a]$, and let $h(x)=1-x^2$, with $a>0$.
The ambient input space is $\R$, while the applied inputs have diameter
$D_{\mathrm{act}}=2a$.
For $\alpha_1(h)=\kappa h$, $\kappa>0$, the ordinary CBF condition is
\begin{equation}\label{eq:examplepsi}
 \psi(x,u)=-2xu+\kappa(1-x^2),\qquad \Ssafe=[-1,1].
\end{equation}
For this illustration, take the exact barrier certificate
$\underline\psi(x,u)=\psi(x,u)$.
For all segments of length at most $\delta_0$ starting in $\Ssafe$,
$|x(s)|\le1+a\delta_0$. Since
$\dot\psi=-2u^2-2\kappa xu$, a valid certificate is $M_\psi=2a^2+2\kappa a(1+a\delta_0)$.\\
% \begin{equation}\label{eq:examplecert}
%  M_\psi=2a^2+2\kappa a(1+a\delta_0).
% \end{equation}
Also, maximizing~\eqref{eq:examplepsi} over inputs $u$ satisfying the actuator constraints gives
$2a|x|+\kappa(1-x^2)$. This is concave as a function of $|x|\in[0,1]$,
so $m_{\mathrm{act}}=\min\{\kappa,2a\}>0$. Proposition~\ref{prop:period} applies when
\begin{equation}\label{eq:exampleperiod}
 \delta\le\delta_0,\qquad
 \delta<\frac{\min\{\kappa,2a\}}
                   {2a^2+2\kappa a(1+a\delta_0)}.
\end{equation}

For $a=1/2$, $\kappa=1$, and $\delta_0=2$, this gives
$M_\psi=5/2$, $m_{\mathrm{act}}=1$, and $\delta<0.4$. Figure~\ref{fig:support}
shows the safe control sets for $\delta=0.1$ and $0.3$. At $x=0.9$, the
instantaneous CBF-based safe control set permits $u\le0.1056$, whereas the respective sampling-period-dependent
safe control sets require $u\le-0.0333$ and $u\le-0.3111$.
The longer hold requires a larger inward safety margin.
\begin{figure}[H]
 \centering
 \includegraphics[width=\columnwidth]{figures/action_support.pdf}
 \caption{Safe control sets within the actuator limits for the scalar example. The unshaded
 region is excluded; longer sampling periods shrink the safe control set.}
 \label{fig:support}
\end{figure}

The effect of zero-order-hold implementation can be seen directly: at $x_0=0.9$, $u=0.1$ gives
$\psi(x_0,u)=0.01\ge0$, but a sampling interval of length $2$ produces
$x(t)=0.9+0.1t>1$ for $t>1$. The sampling-period condition excludes this choice of input and interval. For this plant, the exact safe control set over the sampling interval is
\begin{equation}\label{eq:exactset}
 \U_{\mathrm{act}}\cap\left[\frac{-1-x}{\delta},\frac{1-x}{\delta}\right],
\end{equation}
because the sample-and-hold trajectory is linear in time. It can be much larger than
$\Cdel(x)$; the derivative-margin certificate trades performance freedom for
a simple sufficient safety condition. The example verifies feasibility and quantifies the dependence of the
safe control set on the sampling period.


==> sections/convergence_proof.tex <==
\section{Proof of Theorem~\ref{thm:optimality}}
\label{app:convergence-proof}
Let $\mathcal F_j$ contain all randomness before batch $j$, so
$\theta_j$ is $\mathcal F_j$-measurable. Independent calls to
\textsc{SafeGrad} and Lemma~\ref{lem:variance} give
\begin{equation}\label{eq:batch}
\begin{aligned}
 \E[\overline g_j\mid\mathcal F_j]&=\nabla J_\delta(\theta_j),\\
 \E[\norm{\overline g_j-\nabla J_\delta(\theta_j)}^2
       \mid\mathcal F_j]&\le V_\delta/B.
\end{aligned}
\end{equation}
For $\eta\le L_\delta^{-1}$, smoothness and~\eqref{eq:batch} yield
\begin{equation}\label{eq:ascent}
\begin{aligned}
 \E[J_\delta(\theta_{j+1})\mid\mathcal F_j]
 &\ge J_\delta(\theta_j)
   +\frac\eta2\norm{\nabla J_\delta(\theta_j)}^2\\
 &\quad-\frac{L_\delta\eta^2V_\delta}{2B}.
\end{aligned}
\end{equation}
Define $z_j=J_\delta^*-\E[J_\delta(\theta_j)]-b_\delta$,
$c=\eta/(2a_\delta^2)$, and $d=L_\delta\eta^2V_\delta/(2B)$.
Write $[z]_+=\max\{z,0\}$.
Weak gradient dominance and Jensen's inequality imply
$\E[\norm{\nabla J_\delta(\theta_j)}^2]
\ge[z_j]_+^2/a_\delta^2$, hence
\begin{equation*}
 z_{j+1}\le z_j-c[z_j]_+^2+d.
\end{equation*}
Write
\begin{equation}\label{eq:lambda}
 r=\sqrt{d/c}=a_\delta\sqrt{\frac{L_\delta\eta V_\delta}{B}},
 \qquad \lambda=cr.
\end{equation}
The step-size restriction gives $0<\lambda\le1/2$.
For $z_j\le r$, the recursion gives $z_{j+1}\le r$:
for $z_j\le0$ use $d=\lambda r\le r$, and on $[0,r]$
use monotonicity of $z-cz^2+d$. For $z_j>r$,
\begin{equation*}
 z_j-cz_j^2+d
 =r+(1-2\lambda)(z_j-r)-c(z_j-r)^2.
\end{equation*}
Thus $[z_{j+1}-r]_+\le(1-\lambda)[z_j-r]_+$.
Iteration and $[z_0-r]_+\le p_0$ prove~\eqref{eq:gap}.

For the accuracy guarantee, \eqref{eq:eta} gives
$r\le\varepsilon/2$. Set
\begin{equation}\label{eq:iterations}
 T=\max\left\{1,
      \left\lceil\frac{\Lambda_\varepsilon}{\lambda}\right\rceil
      \right\}.
\end{equation}
Since $(1-\lambda)^T p_0\le\varepsilon/2$,
\eqref{eq:gap} gives $b_\delta+\varepsilon$ accuracy.
Also, $N_{\rm PG}=BT\le B+B\Lambda_\varepsilon/\lambda$;
substitution of~\eqref{eq:eta} proves~\eqref{eq:complexity}.
Equation~\eqref{eq:H} gives the expected interaction count.
A known upper bound may replace $p_0$; by~\eqref{eq:returnbound},
$2\bar r/(1-\gamma)$ is valid. Positive upper bounds on
$L_\delta,V_\delta$ may be used if either original bound is zero.

\begin{remark}[Stationarity without weak gradient dominance]
\label{rem:stationarity}
Under Assumptions~\ref{ass:safety} and~\ref{ass:policy} and the
period condition~\eqref{eq:period}, suppose the iterates remain
in $\Theta$ almost surely. For $0<\eta\le L_\delta^{-1}$ and
integer $T\ge1$, telescoping~\eqref{eq:ascent} yields
\begin{equation}\label{eq:stationary}
\begin{aligned}
 \frac1T\sum_{j=0}^{T-1}\E[\norm{\nabla J_\delta(\theta_j)}^2]
 &\le\frac{2[J_\delta^*-J_\delta(\theta_0)]}{\eta T}\\
 &\quad+\frac{L_\delta\eta V_\delta}{B}.
\end{aligned}
\end{equation}
This uses smoothness,~\eqref{eq:batch}, and
$\E[J_\delta(\theta_T)]\le J_\delta^*$; it does not require
the weak-gradient-dominance inequality~\eqref{eq:gd}.
\end{remark}


==> sections/preamble.tex <==
\usepackage{amsmath,amssymb,mathtools}
% ieeeconf provides a proof environment; let amsthm supply its own consistently.
\let\proof\relax
\let\endproof\relax
\usepackage{amsthm}
\usepackage{graphicx,booktabs,cite}
\usepackage{balance}
\usepackage{float}
\let\labelindent\relax
\usepackage{enumitem}
\floatstyle{ruled}
\newfloat{algorithm}{tbp}{loa}
\floatname{algorithm}{Algorithm}
\usepackage[hidelinks]{hyperref}
\hypersetup{pdftitle={SafePG with Hard Intersample Safety Guarantees},
 pdfauthor={Vipul K. Sharma, Wesley A. Suttle, S. Sivaranjani}}
\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{assumption}[theorem]{Assumption}
\theoremstyle{remark}
\newtheorem{remark}[theorem]{Remark}
% Arabic section prefixes for results; retain lettered appendix prefixes.
\renewcommand{\thetheorem}{\arabic{section}.\arabic{theorem}}
\makeatletter
\g@addto@macro\appendices{%
  \renewcommand{\thetheorem}{\thesection.\arabic{theorem}}%
}
\makeatother
\newcommand{\R}{\mathbb R}
\newcommand{\E}{\mathbb E}
\newcommand{\U}{\mathcal U}
\newcommand{\Ssafe}{\mathcal S}
\newcommand{\Cdel}{\mathcal C_\delta}
\newcommand{\pdel}{\pi_\theta^\delta}
\DeclarePairedDelimiter{\norm}{\lVert}{\rVert}
\DeclarePairedDelimiter{\abs}{\lvert}{\rvert}
\newcommand{\Geom}{\operatorname{Geom}}
\newcommand{\diam}{\operatorname{diam}}
\newcommand{\Pp}{\mathbb{P}}
\usepackage{algpseudocode}


==> sections/related_work.tex <==
\subsection{Related work}
Predictive safety filters~\cite{wabersich2021predictive} use model-based
prediction to enforce constraints; the broader safety-filter literature
distinguishes certification assumptions from the nominal learning
method~\cite{hsu2024filter}. Reduced policy
optimization~\cite{ding2023reduced} combines action reconstruction, implicit
differentiation, and projection to handle hard constraints. Log-barrier
methods~\cite{usmanova2024log} study feasibility-preserving black-box
optimization. These approaches explicitly incorporate constraints or intervention into
policy optimization.

Sample-and-hold CBF analysis~\cite{bahati2023samplehold} and zero-order
CBFs~\cite{tan2025zeroorder} further address sampled execution. Our contribution integrates these safety principles with truncated-policy
learning and finite-sample performance analysis.

PG complexity depends on objective regularity and gradient-estimator
moments~\cite{yuan2022general}. Global performance conclusions require
additional policy or objective structure~\cite{agarwal2021theory}, such as
LQR geometry~\cite{fazel2018global} or weak gradient
dominance~\cite{montenegro2024learning}. We assume the required geometry for the sampled objective and retain its
additive residual; state safety does not establish optimization geometry.

